SoftNeuro: Fast Deep Inference using Multi-platform Optimization

Faster inference of deep learning models is highly demanded on edge devices and even servers, for both financial and environmental reasons. To address this issue, we propose SoftNeuro, a novel, high-performance inference framework with efficient performance tuning. The key idea is to separate algorithmic routines from network layers. Our framework maximizes the inference performance by profiling various routines for each layer and selecting the fastest path. To efficiently find the best path, we propose a routine-selection algorithm based on dynamic programming. Experiments show that the proposed framework achieves both fast inference and efficient tuning.

==> related_works.tex <==
\section{Related Works}
\label{related_works}

A deep learning model consists of a number of convolutional layers and other layers.
A typically used 2D convolutional layer is represented as follows with $I_{y,x}[c]$ as input, $O_{y,x}[c']$ as output, and $W_{ky,kx}[c, c']$ as kernel
\begin{equation}
O_{y,x}[c'] = \sum_{ky,kx,c}{I_{y+ky,x+kx}[c]W_{ky,kx}[c, c']}
\end{equation}
Since most of model inference time is consumed by this convolution operation, it is essential to calculate it efficiently.

There are various approaches to speed up CNNs, such as: Schedule automation, algorithmic speedup (Winograd's algorithm), speedup using sparsity and quantization.

\subsection{Schedule automation}
In order to make the most of the performance of the multiply-accumulator unit used in convolutional operations, it is important to have a memory access pattern that efficiently loads data into the product-accumulator.
Specifically, it is necessary to appropriately set how calculations should be divided and in which order they should be executed (scheduling), and how the multiplier should be loaded and used, at the register level.
However, the best computation method depends on hardware and input/output characteristics (such as data sizes), making it challenging to choose the best method.
Basically, most inference frameworks select a specific computation method by heuristically deciding from the above information. \cite{tensorflowlite, mnn}
Recently, frameworks such as Halide \cite{halide} and TVM \cite{tvm} have adopted an approach where scheduling can be set independently from the content of the computation to optimize it.
Halide \cite{halide} uses a heuristic algorithm (genetic algorithm) to search, \cite{adams2019optimizehalide} restricts scheduling to grouping layers and tiling within them, and uses cache size to determine tile size.
TVM \cite{tvm} adopts the approach of separating algorithm and scheduling, and, at the same time, enables optimization on various hardwares by making it possible to implement the innermost loop of convolutional computation in each hardware (tensorization).
In addition, the optimization of the computation method is predicted by XGBoost \cite{xgboot} based on features such as access to various memories read from IR, which enables efficient search. 
While these methods can optimize model inference as a whole, the number of scheduling combinations is quite large, so limiting the scheduling space and improving the efficiency of search are important issues.

\subsection{Algorithmic speedup (Winograd's algorithm)}
Instead of performing computations as defined, it is known that the total computation volume can be reduced by converting the input and output into different spaces, as Winograd's minimal filtering \cite{winograd} does.
Winograd's method was proposed as a method to minimize the number of multiplications in convolution in the context of digital signal processing, but it can also be extended to convolution in CNN (Convolutional Neural Network) \cite{lavingray2015}, and has been implemented in various inference frameworks. 
As Winograd's method simultaneously calculates convolution over tiles for a specific tile size, choosing the optimal tile size is necessary to improve performance.
Some inference frameworks infer the appropriate tile size based on input characteristics, such as data sizes. \cite{mnn}
Winograd's problem is sometimes limited to the case where stride is 1 and the kernel size is relatively small, but other methods have been devised, such as decomposing the input into smaller kernels and splitting the input into smaller kernels, which leads to the case where stride is 1. 
% splitting the input and decomposing the input, what's the difference?

\subsection{Speedup using sparsity}
CNNs are known to have a large number of zero elements in both the kernel and the intermediate tensor. % are they? citation?
This means computation can be accelerated by explicitly calculating only the non-zero elements.
However, since this calculation is incorporated into SIMD calculation, gather & scatter operations are inevitable, which are not easy to implement efficiently. 
% this calculation is incorporated into SIMD calculation
% what calculation is incorporated into what SIMD calculation? unclear
It is known that the number of zero elements can be further increased depending on the network structure and learning method. % is it? citation?
A common approach to sparse kernels is to score the weights of the kernel and set the lower ones to zero for retraining. \cite{blalock2020}
Group convolution (convolution in which only channels in a particular set are coupled) can also be considered as a kind of sparsity of the kernel, and is often used as an example of sparsity.
In fact, kernels that can run on group convolution can be learned by applying group gruning and group lasso. \cite{huang2018}
Taking into account that there are many zero elements in intermediate tensors \cite{kurtz2020} allows for effective use of SIMD and speeds up inference by using channels last representation and compressed row storage (CRS).

\subsection{Quantization}
% DNNのモデルサイズの削減と計算コスト削減のためにweightやactivationの量子化もよく使用される手法である。
% 量子化は、通常浮動小数点数として扱われる値を整数と少数のパラメータで表現する手法のことで次のような式で表される。
% q = offset + round(x / scale)
% ここでoffsetは整数、scaleは実数である。
% これらの係数の決定方式には複数あり、offsetが0の場合はsymmetricな量子化と呼ばれ、そうではない場合はasymmetricな量子化と呼ばれる。
% また、テンソル毎にquantizeを行うか、channel毎にquantizeを行うかによって精度とモデルサイズのトレードオフが生じる。
% また学習ずみモデルを量子化するpost-quantizationだけでなく、tensorflowなど一部の学習フレームワークでは精度を担保するためにquantization-aware trainingの仕組みも導入されている。
% さらにはweight, activationをa few bitsまで低減したTernary weight networks, Binary Neural Networks, XNOR-net なども提案されているが現在の手法は精度へのインパクトが大きい。

Quantization of weights and activations is another commonly used method to reduce the model size and computational cost of DNNs.
Quantization is a method of expressing a value, which is usually a floating-point number, as an integer and a small number of parameters, via the following equation;

\begin{equation}
q = c + {\rm round}(x / s)
\end{equation}

Where $c$ is an integer offset, and $s$ is a scale.
There are several ways to determine these coefficients: if the offset is zero, it is called symmetric quantization; otherwise, it is asymmetric.
There is also a trade-off between accuracy and model size depending on whether quantization is done per tensor or per channel. % is there? why? citation needed
In addition to post-training quantization, some training frameworks such as TensorFlow \cite{tensorflow2016} have introduced a quantization-aware training mechanism to ensure accuracy \cite{krishnamoorthi2018quantizing}.
Moreover, Ternary weight networks \cite{Li2016TernaryWN}, Binary Neural Networks \cite{Courbariaux2016BinarizedNN},
and XNOR-net \cite{Rastegari2016XNORNetIC}, which reduce the weight and activation to a few bits, have also been proposed.

